Provable Benefit of Random Permutations over Uniform Sampling in Stochastic Coordinate Descent

We analyze the convergence rates of two popular variants of coordinate descent (CD): random CD (RCD), in which the coordinates are sampled uniformly at random, and random-permutation CD (RPCD), in which random permutations are used to select the update indices. Despite abundant empirical evidence that RPCD outperforms RCD in various tasks, the theoretical gap between the two algorithms' performance has remained elusive. Even for the benign case of positive-definite quadratic functions with permutation-invariant Hessians, previous efforts have failed to demonstrate a provable performance gap between RCD and RPCD. To this end, we present novel results showing that, for a class of quadratics with permutation-invariant structures, the contraction rate upper bound for RPCD is always strictly smaller than the contraction rate lower bound for RCD for every individual problem instance. Furthermore, we conjecture that this function class contains the worst-case examples of RPCD among all positive-definite quadratics. Combined with our RCD lower bound, this conjecture extends our results to the general class of positive-definite quadratic functions.

==> temp.tex <==
% Temporary Stuff %

\section*{Temporary Stuff (To be removed)}

Jan 13 Meeting
\begin{itemize}
    \item Why is this problem hard? (Than it seems? Justify our seemingly overspecific, easy-looking problem setting) $\leftrightarrow$ Survey on previous work, no known (theoretical) gap between RCD and RPCD... (story making)
    \item Paper outline (sections, contents)... Sec 3 (RCD, RPCD, provable gap) + Sec 4 (conjecture about why PI is the worst case, maybe for low-dimensional cases like $n = 2, 3$... We have an easy proof for $n = 2$, but $n \ge 3$ is hard.)
    \item About the gap... especially for the large $\sigma$ regime, better if we can show a `positive' gap (if possible)
    \item Include desmos illustrations in the main text... maybe at the end of Sec 3. Visualize how the upper/lower bounds look (ex. show the `bumps' and insist that this makes the analysis hard, use as a visual reference in the proofs, etc...)
\end{itemize}

Jan 23 Meeting
\begin{itemize}
    \item Change notations $T, K$
    \item Motivation... Show real experiments running RCD and RPCD for a certain instance

    (Maybe PI in Section 1, non-PI examples in the experiment section, plus analyze and compare with our theorems)
\end{itemize}
